Permissible Knowledge Pooling

Information pooling has been extensively formalised across various logical frameworks in distributed systems, characterized by diverse information-sharing patterns. These approaches generally adopt an intersection perspective, aggregating all possible information, regardless of whether it is known or unknown to the agents. In contrast, this work adopts a unique stance, emphasising that sharing knowledge means distributing what is known, rather than what remains uncertain. This paper introduces new modal logics for knowledge pooling and sharing, ranging from a novel language of knowledge pooling to a dynamic mechanism for knowledge sharing. It also outlines their axiomatizations and discusses a potential framework for permissible knowledge pooling.

==> TabFig/fig_RG.tex <==
\tikz[every lower node part/.style={black}] {
  \begin{scope}[name prefix = 2-]
    \node [circle split,draw, minimum size=1.2cm] (0) at (0,0) {$s_0$ \nodepart{lower} $p,q,r$};
 %   \node [circle split,draw, minimum size=1.2cm] (1) at (-2.5,1) {$s_1$ \nodepart{lower} $p,\neg q,  r$};
    \node [circle split,draw, minimum size=1.2cm] (1) at (-2.5,0) {$s_1$ \nodepart{lower} $p,\neg q,  \neg r$};
    \node [circle split,draw, minimum size=1.2cm] (2) at (2.5,0) {$s_2$ \nodepart{lower} $ p,  q, \neg r$};
    \path[draw, dashed] 
    (0) edge node[above, name=a] {$a$} (1)
    (0) edge node[above, name=a] {$a,b$} (2); 
 %   (0) edge node[below, name=b] {$b$} (3);
  \end{scope}
}

==> TabFig/fig_S0.tex <==
\tikz[every lower node part/.style={red}] {
  \begin{scope}[name prefix = 1-]
    \node [circle split,draw, minimum size=1.2cm] (A) at (0,0) {$s_0$ \nodepart{lower} $p$};
  \end{scope}
  \begin{scope}[name prefix = 2-]
    \node [circle split,draw, minimum size=1.2cm] (A) at (3,0) {$s_1$ \nodepart{lower} $p,q$};
    \node [circle split,draw, minimum size=1.2cm] (B) at (1.5,2) {$s_2$ \nodepart{lower} $\neg p, q$};
    \node [circle split,draw, minimum size=1.2cm] (C) at (4.5,2) {$s_3$ \nodepart{lower} $\neg p, \neg q$};
    \path[draw, dashed] 
    (A) edge node[above, name=b] {$b$} (B)
    (B) edge node[above, name=b] {$b$} (C) 
     (C) edge node[above, name=b] {$b$} (A);
  \end{scope}
  \begin{scope}[name prefix = 3-]
    \node [circle split,draw, minimum size=1.2cm] (A) at (6,0) {$s_4$ \nodepart{lower} $p,q,r$};
    \node [circle split,draw, minimum size=1.2cm] (B) at (4.5,-2) {$s_5$ \nodepart{lower} $p,\neg q, r$};
    \node [circle split,draw, minimum size=1.2cm] (C) at (7.5,-2) {$s_6$ \nodepart{lower} $p,\neg q, \neg r$};
    \path[draw, dashed] 
    (A) edge node[above, name=c] {$c$} (B)
    (B) edge node[above, name=c] {$c$} (C)
    (C) edge node[above, name=c] {$c$} (A);
  \end{scope}

  \draw [red,dashed] (1-A) edge node[above, name=a]  {$a$} (2-A);
  \draw [red,dashed] (2-A) edge node[above, name=b] {$b$} (3-A);
}

==> TabFig/fig_S1.tex <==
\tikz[every lower node part/.style={red}] {
  \begin{scope}[name prefix = 1-]
    \node [circle split,draw, minimum size=1.2cm] (A) at (0,0) {$s_0$ \nodepart{lower} $p$};
  \end{scope}
  \begin{scope}[name prefix = 2-]
    \node [circle split,draw, minimum size=1.2cm] (A) at (3,0) {$s_1$ \nodepart{lower} $p,q$};
    \node [circle split,draw, minimum size=1.2cm] (B) at (1.5,2) {$s_2$ \nodepart{lower} $\neg p, q$};
    \node [circle split,draw, minimum size=1.2cm] (C) at (4.5,2) {$s_3$ \nodepart{lower} $\neg p, \neg q$};
    \draw[dashed]  (B) edge node[above, name=b] {$b$} (C)  ;
  \end{scope}
  \begin{scope}[name prefix = 3-]
    \node [circle split,draw, minimum size=1.2cm] (A) at (6,0) {$s_4$ \nodepart{lower} $p,q,r$};
    \node [circle split,draw, minimum size=1.2cm] (B) at (4.5,-2) {$s_5$ \nodepart{lower} $p,\neg q, r$};
    \node [circle split,draw, minimum size=1.2cm] (C) at (7.5,-2) {$s_6$ \nodepart{lower} $p,\neg q, \neg r$};
    \path[draw, dashed] 
    (A) edge node[above, name=c] {$c$} (B)
    (B) edge node[above, name=c] {$c$} (C)
    (C) edge node[above, name=c] {$c$} (A);
  \end{scope}

  \draw [red,dashed] (1-A) edge node[above, name=a]  {$a$} (2-A);
  \draw [red,dashed] (2-A) edge node[above, name=b] {$b$} (3-A);
}

==> appx.tex <==
  


\begin{lemma} %\label{lem:update}
Let $M|_{a \smalltriangleright b} = \langle W,  \{R^*_i\}_{i \in \mathcal{I}}, V\rangle$ be a $(a \smalltriangleright b)$-updated model. 
\begin{enumerate}
     \item $M|_{a \smalltriangleright b}$ is still a model.  %\label{lem:u2}
   \item Let $Prop^+$ be the set of Boolean propositions that only construct from atomic propositions, negation, and conjunction. 
        $$uR^*_bs \textrm{ iff } uR_b s \textrm{ and } \forall \phi \in K_a^+ u\, (u \in || \phi||_M \Leftrightarrow s \in  ||\phi||_M)$$
        where $K_a^+ u = \{ \phi \in Prop^+ \mid M, u \models K_a \phi\}$.  %\label{lem:u1} 
    \item Let $u \in W$. So, $M, u \models \phi$ iff $M|_{a\smalltriangleright b}, u\models \phi$, where $\phi \in Prop^+$. %\label{lem:u3}
    \item $R_a \cap R_b \subseteq R^*_b$.%\label{lem:u4}
    \item $D_G = D_G^*$.%\label{lem:u5}
\end{enumerate}
\end{lemma}
\begin{proof}
\begin{enumerate}
    \item We only need to show that $R^*_b$ is still an equivalent relation. 
\begin{itemize}
    \item Reflexivity: Due to the reflexivity of $R_b$ we have $uR_bu$ where any $u \in R_b[w]$. Due to Definition~\ref{def:update}.\ref{def:u2}, it is obvious that the bi-direction holds. So $uR^*_bu$ for any $u\in W$.

    \item Transitivity: Given $uR^*_bs$ and $sR^*_bv$, we know that $uR_bs$ and $sR_bv$. So we have $uR_bv$ because of the transitivity of $R_b$. According to the bi-direction in Definition~\ref{def:update}.\ref{def:u2}, it is the case that $\forall p \in K_a u(u \in ||p||_M \Leftrightarrow v\in ||p||_M)$. Now we have $uR^*_bv$. 
    \item Symmetry: Let $uR^*_bs$. So $uR_bs$. According to the bi-equivalence of Definition~\ref{def:update}.\ref{def:u2}, it is not hard to imply $\forall p\in K_a s\,(s \in ||p||_M \Leftrightarrow u\in ||p||_M)$. This obviously leads to $uR^*_bs$.  
\end{itemize}

    \item We only need to show that from $uR^*_bs$ we can have the bi-direction for all formulas in $K_a^+w$. This can be proven by inducing on the complexity of formulas in $Prop^+$ in a standard way. 


\item Inducing on the complexity of $Prop^+$. 
\begin{itemize}
    \item Basic case: When $\phi = p \in Prop$, this bi-equivalence holds by the definition of the valuation function in $M|_{a \smalltriangleright b}$. 
    \item Induction hypothesis: Given a subformula $\psi \in Prop^+$ of $\phi$, the bi-equivalence for $\psi$ holds. 
    \item Now the other cases such as either $\phi = \neg\psi$ or $\phi = \psi \wedge \psi'$ can easily be proven due to the induction hypothesis in a standard way.
\end{itemize}

\item This is obvious by Definition~\ref{def:update}.\ref{def:u2}.
\item This can be shown by the set-theoretic feature that both $D_G$ and $D^*_G$ are obtained by intersection.
\end{enumerate}
\end{proof}

==> old/appx_old.tex <==
\begin{lemma} %\label{lem:update}
Let $M|_{a \smalltriangleright b} = \langle W,  \{R^*_i\}_{i \in \mathcal{I}}, V\rangle$ be a $(a \smalltriangleright b)$-updated model. 
\begin{enumerate}
     \item $M|_{a \smalltriangleright b}$ is still a model.  \label{lem:u2}
   \item \label{lem:u1} Let $Prop^+$ be the set of Boolean propositions that only construct from atomic propositions, negation, and conjunction. 
        $$uR^*_bs \textrm{ iff } uR_b s \textrm{ and } \forall \phi \in K_a^+ u\, (u \in || \phi||_M \Leftrightarrow s \in  ||\phi||_M)$$
        where $K_a^+ u = \{ \phi \in Prop^+ \mid M, u \models K_a \phi\}$. 
    \item Let $u \in W$. So, $M, u \models \phi$ iff $M|_{a\smalltriangleright b}, u\models \phi$, where $\phi \in Prop^+$. \label{lem:u3}
    \item $R_a \cap R_b \subseteq R^*_b$.\label{lem:u4}
    \item $D_G = D_G^*$.\label{lem:u5}
\end{enumerate}
\end{lemma}
\begin{proof}
\begin{enumerate}
    \item We only need to show that $R^*_b$ is still an equivalent relation. 
\begin{itemize}
    \item Reflexivity: Due to the reflexivity of $R_b$ we have $uR_bu$ where any $u \in R_b[w]$. Due to Definition~\ref{def:update}.\ref{def:u2}, it is obvious that the bi-direction holds. So $uR^*_bu$ for any $u\in W$.

    \item Transitivity: Given $uR^*_bs$ and $sR^*_bv$, we know that $uR_bs$ and $sR_bv$. So we have $uR_bv$ because of the transitivity of $R_b$. According to the bi-direction in Definition~\ref{def:update}.\ref{def:u2}, it is the case that $\forall p \in K_a u(u \in ||p||_M \Leftrightarrow v\in ||p||_M)$. Now we have $uR^*_bv$. 
    \item Symmetry: Let $uR^*_bs$. So $uR_bs$. According to the bi-equivalence of Definition~\ref{def:update}.\ref{def:u2}, it is not hard to imply $\forall p\in K_a s\,(s \in ||p||_M \Leftrightarrow u\in ||p||_M)$. This obviously leads to $uR^*_bs$.  
\end{itemize}

    \item We only need to show that from $uR^*_bs$ we can have the bi-direction for all formulas in $K_a^+w$. This can be proven by inducing on the complexity of formulas in $Prop^+$ in a standard way. 


\item Inducing on the complexity of $Prop^+$. 
\begin{itemize}
    \item Basic case: When $\phi = p \in Prop$, this bi-equivalence holds by the definition of the valuation function in $M|_{a \smalltriangleright b}$. 
    \item Induction hypothesis: Given a subformula $\psi \in Prop^+$ of $\phi$, the bi-equivalence for $\psi$ holds. 
    \item Now the other cases such as either $\phi = \neg\psi$ or $\phi = \psi \wedge \psi'$ can easily be proven due to the induction hypothesis in a standard way.
\end{itemize}

\item This is obvious by Definition~\ref{def:update}.\ref{def:u2}.
\item This can be shown by the set-theoretic feature that both $D_G$ and $D^*_G$ are obtained by intersection.
\end{enumerate}
\end{proof}

\begin{proposition} %\label{prop:main}
Here are some validities about the update of $a \smalltriangleright b$:
\begin{enumerate}
     \item A: $[a \smalltriangleright b] p \leftrightarrow p$
     \item C: $[a \smalltriangleright b](\varphi \wedge \psi)\leftrightarrow [a \smalltriangleright b]\varphi \wedge [a \smalltriangleright b]\psi$, where $\varphi,\psi \in \mathcal{L}$
     \item N: $[a \smalltriangleright b]\neg\varphi \leftrightarrow \neg[a \smalltriangleright b]\varphi$ for any $\varphi \in \mathcal{L}$
   \item \label{prop:m1} $U_1$: $K_a \phi \to [a \smalltriangleright b]K_b \phi$, where $\phi \in Prop^+$
    \item \label{prop:m2} $U_2$: $K_b\phi \to [a\smalltriangleright b]K_b\phi$ for $\phi \in \mathcal{L}$
    \item \label{prop:m3} $U_3$: $K_c\phi \to [a\smalltriangleright b]K_c\phi$ where $\phi \in \mathcal{L}$ and $c \neq b$
    \item \label{prop:m4} $U_4$: $[a\smalltriangleright b] K_b\varphi \to D_{\{a,b\}}[a\smalltriangleright b]\varphi$ where $\varphi \in \mathcal{L}$
    \item \label{prop:md} $U_5$: $[a\smalltriangleright b] D_G\varphi \leftrightarrow D_G[a\smalltriangleright b]\varphi$ where $\varphi \in \mathcal{L}$

   \item K-axiom: $[a\smalltriangleright b](\phi \to \psi) \to ([a\smalltriangleright b]\phi \to [a\smalltriangleright b] \psi)$ where $\varphi,\psi \in \mathcal{L}$  
    \item \label{prop:nec} NEC Rule: If $\vdash \phi$ then $\vdash [a\smalltriangleright b]\phi$ where $\varphi \in \mathcal{L}$

\end{enumerate}
\end{proposition}
\begin{proof}
\begin{enumerate}
\item The truth condition for atomic propositions is never changed, according to Definition~\ref{def:update}.
\item This can be proved by using Definition~\ref{def:update} many times. 
\item The negation about pooling behaves in this way:
\begin{align*}
    M, w \models \neg [a\smalltriangleright b]\varphi &\textrm{ iff } M, w \not\models [a\smalltriangleright b]\varphi \\
    & \textrm{ iff }  M|_{a\smalltriangleright b}, w \not\models\varphi\\
    & \textrm{ iff }  M|_{a\smalltriangleright b}, w \models\neg\varphi\\
    & \textrm{ iff } M, w \models [a\smalltriangleright b]\neg\varphi.
\end{align*}

\item Let $M, w \models K_a \phi$ and $wR^*_b u$ in the updated model $M|_{a\smalltriangleright b}$, where $\phi \in Prop^+$. We need to show that $M|_{a\smalltriangleright b}, u \models \phi$. According to Lemma~\ref{lem:update}.\ref{lem:u1} and $wR^*_b u$, we know that $\forall \phi \in K_a^+ w\,( w \in ||\phi||_M \Leftrightarrow u \in ||\phi||_M)$ (@). From $M, w \models K_a \phi$ and T-axiom, we know that $M, w \models \phi$. Then, by (@), it implies that $M, u \models \phi$. Then, due to Lemma~\ref{lem:update}.\ref{lem:u3}, we conclude that $M|_{a\smalltriangleright b}, u \models \phi$. 

\item This axiom is valid because $R_b^* \subseteq R_b$ by Definition~\ref{def:update}.\ref{def:u2}.

\item This axiom is valid because $R^*_a = R_a$ by Definition~\ref{def:update}.\ref{def:u1}.

\item This can be demonstrated by using Lemma~\ref{lem:update}.\ref{lem:u4}.

\item This can be shown by using Lemma~\ref{lem:update}.\ref{lem:u5}. 

\item As Lemma~\ref{lem:update}.\ref{lem:u2} demonstrated, after a $(a\smalltriangleright b)$-update, the structure $M|_{a\smalltriangleright b}$ is still a model. It therefore concludes $\psi$ being true at $w$, when $\phi \to \psi$ and $\phi$ are both satisfied at the same point $w$ in the updated model $M|_{a\smalltriangleright b}$. 

\item If $\phi$ is true everywhere in the model, then it simply ensures it is always true at both sides of the bi-direction in Definition~\ref{def:update}.\ref{def:u2} for every pair of worlds. This indicates that, after any $(a\smalltriangleright b)$-update, $\phi$ is still true everywhere in the updated model. 
\end{enumerate}
\end{proof}



\begin{proposition} %\label{prop:3par}
    The following validities clarify the transitions of knowledge pooling from one agent towards the third party:
\begin{enumerate}
    \item \label{prop:tran} $[a\smalltriangleright b][b\smalltriangleright c]K_c\varphi \to [a\smalltriangleright c]K_c\varphi$ where $\varphi \in Prop^+$
    \item \label{prop:m5} $[a\smalltriangleright b]K_b \phi \to [a \smalltriangleright b][b\smalltriangleright c]K_c \phi$, where $\phi \in Prop^+$
\end{enumerate}
\end{proposition}
\begin{proof}
\begin{enumerate}
\item First of all, in a $(a\smalltriangleright b)$-model $M$, it has $K^+_bw|_{a\smalltriangleright b} = Cn(K^+_bw \cap K^+_aw)$. Let $K^+_bw|_{a\smalltriangleright b} = K^+_bw^*$. Similarly, we have $K^+_c(w|_{a\smalltriangleright b})|_{b\smalltriangleright c} = Cn(K^+_cw \cap K^+_bw^*)$ and $K^+_cw|_{a\smalltriangleright c} = Cn(K^+_cw \cap K^+_aw)$. So $K^+_c(w|_{a\smalltriangleright b})|_{b\smalltriangleright c} \subseteq K^+_cw|_{a\smalltriangleright c}$. Together with Lemma~\ref{lem:update}.\ref{lem:u3}, this ensures the desired result. 

\item Let $M, w \models [a\smalltriangleright b]K_b\phi$ where $\phi \in Prop^+$. This is $M|_{a\smalltriangleright b}, w \models K_b\phi$. Because of Proposition~\ref{prop:main}.\ref{prop:m1}, we know that $M|_{a\smalltriangleright b}, w \models K_b\phi \to [b\smalltriangleright c]K_c\phi$. Now we conclude with $M|_{a\smalltriangleright b}, w \models [b\smalltriangleright c]K_c\phi$. This leads to the desired result $M, w\models[a\smalltriangleright b][b\smalltriangleright c]K_c\phi$.
\end{enumerate}
\end{proof}


\begin{proposition}
    \begin{enumerate}
    \item $K_a\phi \to R_GE_G\phi$, where $\phi \in Prop^+$ and $G = \{a, b_1,\dots, b_n\}$.
    \item $R_GE_G\phi \to R^i_GE_G\phi \leftrightarrow D_GR^i_G\phi$, where $\phi \in Prop^+$ and $a\in G$. 
\end{enumerate}
\end{proposition}
\begin{proof}
\begin{enumerate}
    \item We want to prove $K_a\phi \to [a\smalltriangleright b_1]\cdots [b_{n-1}\smalltriangleright b_n][b_n \smalltriangleright b_{n-1}]\cdots[b_1\smalltriangleright a]E_G\phi$. From Proposition~\ref{prop:main}, we have
    \begin{itemize}
        \item $K_a\phi \to [a\smalltriangleright b_1]K_{b_1}\phi$ \\(by Proposition~\ref{prop:main}.\ref{prop:m1})
        \item $[b_n\smalltriangleright b_{n+1}]K_{b_{n+1}}\phi \to [b_n\smalltriangleright b_{n+1}] [b_{n+1}\smalltriangleright b_{n+2}] K_{b_{n+2}}\phi$ \\(by Proposition~\ref{prop:3par}.\ref{prop:m5})
        \item $[b_n\smalltriangleright b_{n+1}]K_{b_{n+1}}\phi \to [b_n\smalltriangleright b_{n+1}][b_{n+1}\smalltriangleright b_{n+2}] K_{b_{n+1}}\phi$ \\(by Proposition~\ref{prop:main}.\ref{prop:m3}, NEC, K, MP)
    \end{itemize}
    And these validities together can lead to the desired result. 
\item First of all, when $b_i \in G$ ($1 \leq i \leq n$)
\begin{align*}
    R_{b_i}|_G = \bigcap_{b\in G} R_b \subseteq R^*_{b_i}
\end{align*}
according to Definition~\ref{def:update}. So the first implication holds. The second bi-direction also holds and its proof can refer to~\cite{aagotnes2017resolving}. 
\end{enumerate}   
\end{proof}



\begin{proposition} %\label{prop:perm}
    Here are some validities:
\begin{enumerate}
    \item \label{prop:o-tran} $[a\smalltriangleright b][b\smalltriangleright c]\hat{K_c}{\sf O} \to [a\smalltriangleright c]\hat{K_c}{\sf O}$
   % \item $P(a\smalltriangleright a)$
    \item \label{prop:3tran}$ P(a\smalltriangleright b) \wedge [a\smalltriangleright b]P(b \smalltriangleright c) \to P(a\smalltriangleright c)$
    \item \label{prop:Keq} If $\vdash K_a\varphi \leftrightarrow K_b \varphi$ then $P(a\smalltriangleright c) \leftrightarrow P(b \smalltriangleright c)$
\end{enumerate}
\end{proposition}
\begin{proof}
\begin{enumerate}
    \item As the proof for Proposition~\ref{prop:3par}.\ref{prop:tran} shown, it is the case that $K_c(w|_{a\smalltriangleright b})|_{b\smalltriangleright c} \subseteq K_cw|_{a\smalltriangleright c}$. By Definition~\ref{def:update}, it ensures that $((R_c)|_{a\smalltriangleright b})|_{b \smalltriangleright c}[w]\subseteq (R_c)|_{a\smalltriangleright c}[w]$, which leads us to the desired result. 
    %\item Let $M, w\models P_a\varphi$. This means $M, w \models K_a\varphi$ and $R_a[w]\cap O[w] \neq \emptyset$. According to Proposition~\ref{prop:main}.\ref{prop:m3}, we have $M|_{a\smalltriangleright b}, w\models K_a\varphi$. Due to Definition~\ref{def:update}.\ref{def:u1}, $R_a^* = R_a$. So $R^*_a[w]\cap O[w] \neq \emptyset$. Both conclusions ensure $M|_{a\smalltriangleright b}, w \models P_a\varphi$. 
    \item Let $M, w \models P(a\smalltriangleright b)$ and $M, w \models [a\smalltriangleright b]P(b\smalltriangleright c)$. This implies
    \begin{itemize}
        \item If $M, w \models K_a\varphi$ then $M|_{a\smalltriangleright b}, w \models P_b\varphi$ for any $\varphi$;
        \item If $M, w \models [a\smalltriangleright b]K_b\varphi$ then $M, w \models [a\smalltriangleright b][b \smalltriangleright c]P_c\varphi$.
        %If $M|_{a\smalltriangleright b}, w \models P_b\varphi$ then $(M|_{a\smalltriangleright b})|_{b\smalltriangleright c}, w \models P_c\varphi$ for any $\varphi$.
    \end{itemize}
So we have
\begin{itemize}
    \item If $M, w \models K_a\varphi$ then $M, w \models [a\smalltriangleright b][b \smalltriangleright c]P_c\varphi$ for any $\varphi$.
\end{itemize}
From Proposition~\ref{prop:3par}.\ref{prop:tran} we have:
\begin{itemize}
    \item $[a\smalltriangleright b][b\smalltriangleright c]K_c\varphi \to [a\smalltriangleright c]K_c\varphi$;
\end{itemize}
While, from Proposition~\ref{prop:perm}.\ref{prop:o-tran} we have
\begin{itemize}
    \item $[a\smalltriangleright b][b\smalltriangleright c]{\sf O}_c \to [a\smalltriangleright c]{\sf O}_c$.
\end{itemize}
These two statements result 
\begin{itemize}
    \item $[a\smalltriangleright b][b\smalltriangleright c]P_c\varphi \to [a\smalltriangleright c]P_c\varphi$.
\end{itemize}
This leads to what we want to prove $M, w \models P(a\smalltriangleright c)$, which is
    \begin{itemize}
        \item If $M, w \models K_a\varphi$ then $M, w \models [a\smalltriangleright c]P_c\varphi$ for any $\varphi$.
    \end{itemize}
\end{enumerate}
\end{proof}

